Combinatorial Optimization of AC Optimal Power Flow with Discrete Demands in Radial Networks

The AC Optimal power flow (OPF) problem is one of the most fundamental problems in power systems engineering. For the past decades, researchers have been relying on unproven heuristics to tackle OPF. The hardness of OPF stems from two issues: (1) non-convexity and (2) combinatoric constraints (e.g., discrete power extraction constraints). The recent advances in providing sufficient conditions on the exactness of convex relaxation of OPF can address the issue of non-convexity. To complete the understanding of OPF, this paper presents a polynomial-time approximation algorithm to solve the convex-relaxed OPF with discrete demands as combinatoric constraints, which has a provably small parameterized approximation ratio (also known as PTAS algorithm). Together with the sufficient conditions on the exactness of the convex relaxation, we provide an efficient approximation algorithm to solve OPF with discrete demands, when the underlying network is radial with a fixed size and one feeder. The running time of PTAS is $O(n^{4m/\epsilon}T)$, where $T$ is the time required to solve a convex relaxation of the problem, and $m, \epsilon$ are fixed constants. Based on prior hardness results of OPF, our PTAS is among the best achievable in theory. Simulations show our algorithm can produce close-to-optimal solutions in practice.

==> nomcl.tex <==
\vspace*{-10pt}
\section*{Nomenclature}

\addcontentsline{toc}{section}{Nomenclature}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{{\sc OPF}}]
\item[]
\hspace{-40pt} Electric Networks
\item[$\cV^+$] Set of nodes in distribution network without root $0$
\item[$\cE$] Set of links in distribution network
\item[$\cE_j$] Set of links of subtree from $j \in \cV$
\item[$(i,j)$] Directed edge, $i$ is a parent of $j$ in a rooted tree
\item[$\cN$]  Set of all users
\item[$\cI$]  Set of users with discrete demands ($s_k \in \{0, \overline s_k \}$)
\item[$\cF$]  \mbox{Set of users with continuous demands ($\underline s_k \le s_k \le \overline s_k$)}
\item[$\cU_j$] Set of users attached to node $j \in \cV$
\item[$\cN_j$] Set of users attached to the subtree from $j \in \cV$
\item[$\cP_j, \cP_k$] Path from root $0$ to node $j$ or user $k$ 

\hspace{-40pt} Parameters
\item[$v_0$] Voltage magnitude square at root $0$
\item[$\overline \ell_{i,j}$] Upper limit of current magnitude sq. through $(i,j)$
\item[$\overline S_{i,j}$] Upper limit of power flow through $(i,j)$
\item[$\overline v_j,\underline v_j $]  Upper \& lower limits of voltage magnitude sq. at $j$
\item[$\overline s_k,\underline s_k$]  Upper \&  lower limits of power demand of user $k$
\item[$f_0(\cdot)$] Cost function of total real power supply
\item[$f_k(\cdot)$] Objective function of real power demand of user $k$
\item[$z_{i,j}$] Impedance of  link $(i,j)$
\item[$\phi$] Maximum difference between the phase angles of any pair of discrete power demands

\hspace{-40pt} Variables
\item[$s_k$]  Power demand of user $k$
\item[$x_k$]  Binary control variable of  discrete demand of $k \in \cI$
\item[$s_0$] Total  power supply (or injection) at root $0$
\item[$\ell_{i,j} $]  Current magnitude sq. through link $(i,j)$
\item[$v_j $]  Voltage magnitude sq. at node $j$
\item[$S_{i,j} $]  Power flow through link  $(i,j)$

%\hspace{-40pt} Acronyms 
%\item[$\textsc{PTAS}$] Polynomial-time approximation scheme
%\item[$\textsc{cOPF}$] Convex-relaxed OPF
%\item[$\textsc{OPF}^\phi$] Rotated OPF by angle $\phi$
\end{IEEEdescription}

